PlexiChain: A Secure Blockchain-based Flexibility Aggregator Framework

Flexible resources in built environments are seen as a low-cost opportunity for delivering grid management services. Consequently, the centralised aggregator model, where the aggregator is used to bundle demand flexibility from flexible resources and deliver it to flexibility customers such as Distributed/Transmission System Operator (DSO/TSO) in flexibility markets, has been adopted. However, the aggregator role introduces various security and trust challenges. In this work, we propose a blockchain-based flexibility trading framework dubbed PlexiChain to address the security and trust challenges the aggregator poses in the centralised aggregator model. The security evaluations performed using a real-world dataset show that PlexiChain is robust against known security attacks, such as MadIoT and False Data Injection attacks. Additionally, the performance evaluations show that PlexiChain has lower computation and communication costs than other blockchain-based applications in resource-constrained environments.

==> sections/2-preliminaries.tex <==
\section{Preliminaries} \label{sec:preliminaries}
In this section, we introduce the NFT and CSP concepts.
Then, in \Cref{sec:plexichain} we use these concepts as building blocks of the proposed PlexiChain framework.

% \subsection{Local Flexibility Markets}
% As shown in \Cref{fig:incentive-based_dr_program}, the LFM includes market participants, flexibility products, and a value chain.
% We give a high-level overview of each concept as follows:

% \subsubsection{Market participants}
% Some of the key participants involved in the LFMs include the Prosumers, Flexible Resources, Aggregators, DSOs, and TSOs \cite{USEF2018}.
% Prosumers are the flexibility suppliers who own flexible resources. 
% Flexible resources consist of energy devices installed in built environments (e.g. HVAC, DERs, EVs and ESS) that can be controlled to provide flexibility services.
% The role of the Aggregator is to accumulate flexibility from the prosumers and sell it to either the DSO or the TSO.
% The DSO and TSO are system operators at the distribution and transmission level respectively.
% Theese entities are responsible for managing electricity from generation sources is distributed to end consumers. DSO are expected to play a more complex role of supporting the two way interactive system involving various Distributed Energy Resources.
% \begin{table}[!tbp]
% \caption{Flexibility Products}
% \begin{center}
% \begin{tabularx}{\linewidth}{|c|l|X|}
% \hline
% \textbf{Flexibility}&\multicolumn{2}{|c|}{\textbf{Aggregated Prosumer Flexibility}} \\
% \cline{2-3} 
% \textbf{Customer} & \textbf{\textit{Flexibility service}}& \textbf{\textit{Flexibility purpose}}\\
% \hline
% Prosumer & Time-of-Use optimisation & Reduce energy cost  \\\cline{2-3}
%  & KWmax control & Reduce grid connection cost  \\\cline{2-3}
%  & Self balancing & Reduce energy cost  \\\cline{2-3}
%  & Controlled Islanding & Increase availability  \\\hline
% DSO & Congestion management & Delay grid reinforcement  \\\cline{2-3}
%  & Voltage control & Avoid grid reinforcement  \\\cline{2-3}
%  & Control Islanding & Reduce frequency and duration of outages  \\\cline{2-3}
%  & Power quality support & Avoid grid investments  \\\hline
% TSO & Congestion management & Delay grid reinforcement  \\\cline{2-3}
%  & Primary control & Maintain system stability and reliability  \\\cline{2-3}
%  & Control Islanding & Reduce frequency and duration of outages  \\\cline{2-3}
%  & Grid capacity management & Optimise assets use  \\\hline
 
% \end{tabularx}
% \label{tab:flexibility_products}
% \end{center}
% \end{table}
% \subsubsection{Flexibility products}
% The aggregator is responsible for acquiring flexibility from prosumers through DR programs such as load shifting, DER generation, and ESS management \cite{Olivella-Rosell2018}.
% A Prosumer can use its own flexibility for in-built optimisation before flexibility is offered to other customers in the energy market.
% The flexibility offered in the energy market varies in shape, quantity and direction depending on the type of flexibility customer, service and purpose \cite{Villar2018}, as summarised in \Cref{tab:flexibility_products}.
% The flexibility service determines the shape, either generation or consumption.
% Also, the quantity can be constrained to the minimum or maximum energy consumption over the time frame considered.
% Lastly, flexibility can be determined by the direction feature, where flexibility can take the form of either increasing or decreasing the consumption or production load.
% In this work, we focus on the flexibility direction to provide the following two types of flexibility products from the prosumers' point of view.
% \begin{itemize}
%     \item \textbf{Positive flexibility ($F^{+VE}$):} This flexibility product requires the prosumers to increase their energy consumption or decrease their local energy production without compromising their own flexibility needs.
%     For example, a prosumer could act as an energy sink by charging their ESS during off-peak hours.
%     \item \textbf{Negative flexibility ($F^{-VE}$):} This flexibility product requires the prosumers to decrease their energy consumption or increase their local production.
%     For example, the prosumer could act as an energy source by discharging their ESS during peak hours.
% \end{itemize}
% \subsubsection{Flexibility trading value chain}
% The flexibility value chain describes the set of activities done by the market participants in order to deliver the flexibility products to the LFMs.
% In \Cref{fig:current_model}, we depict a generic data flow architecture for demand flexibility trading adopted from \cite{Jin2020}.
% The architecture splits the value chain into four abstract layers, which include the grid layer, ICT layer, control layer and the market layer.
% Further, the architecture identifies the participants involve and the set of activities done at each layer.

% \begin{figure} [!th]
%     \centering
%     \includegraphics[width=\linewidth]{figures/PlexiChain-system_model.png}
%     \caption{Load flexibility delivery model}
%     \label{fig:current_model}
% \end{figure}

% The grid layer is composed of all power resources in the smart grid system ranging from transmission and distribution energy resources to flexible DERs.
% These resources are used to generate, transmit and consume electric energy. 
% The ICT layer comprises all computing resources used to collect, transmit, process and store consumption and generation data from the power resources in the grid layer.
% For instance, IoT devices such as smart meters, light sensors, and temperature sensors are used for data collection, routers and gateways are used for data transmission, and edge-fog cloud servers are used for data processing and storage.
% The control layer is composed of the communication and control standards that automate DR.
% The most common communication standard for automating DR is the Open Automated DR (OpenADR) standard \cite{Jin2020}.
% Lastly, the market layer is responsible for the management of flexibility trading.
% Various business models, such as incentive and price based models, have been proposed in the literature to facilitate local flexibility trading.


% \subsection{HARB Framework}
% The HARB framework is a custom Hyperledger Fabric blockchain framework that exploits the rich representation ability of hypergraphs to scale the existing blockchain framework for applications in resource-constrained IoT environments.
% \Cref{fig:plexichain} depicts a generic architecture of the HARB framework adopted from \cite{Karumba2020}.
% The architecture is split into three abstraction layers, which include the underlay (network) layer, the Overlay (consensus) layer, and the control (application) layer.
% Each layer is described as follows:

% \subsubsection{Network layer}
%     The network layer is responsible for inter-node communication.
%     The current blockchain networks are fundamentally based on ordinary graph structures, commonly referred to as peer-to-peer (P2P) networks.
%     Ordinary graphs model the relationship between pairs of nodes in a P2P network using an edge.
%     In contrast, a hypergraph is a generalisation of graphs in which a hyperedge can model a relationship between any number of nodes to create a high-order network \cite{Agarwal2006}.
%     The HARB framework network is composed of an interactions manager and a network clustering manager.
%     The interactions manager uses hyperedges to map out complex high-order relationships in a distributed network rather than the pairwise relationships mapped out by an edge.
%     Consequently, the clustering manager uses the high-order relationships mapped out by the interactions manager to organise nodes into maximally coherent groups or clusters. 
%     Each cluster acts as Sidechain, making the HARB network more scalable.
    
% \subsubsection{Consensus layer}
%     The consensus layer is responsible for validating transactions, ordering them and guaranteeing that everyone agrees on the generated block. 
%     Instead of the widely used order-execute consensus model for transaction execution and validation, the HARB framework uses an execute-order-validate model proposed by IBM researchers \cite{Karandikar2019}.
%     Unlike the order-execute model, where transactions are first ordered and then executed by all nodes, in the execute-order-validate model, transactions are first executed by the minority and then validated by the majority.
%     Nodes that provide an interface to the external users are called the \textit{client (anchor) peers}; the nodes that execute transaction are called \textit{Endorsing peers}; the nodes that orders transactions are called \textit{Ordering peers}; and nodes that validate and store transactions are called the \textit{Committing peers}.
%     In addition, the HARB framework introduces \textit{Notary peers} based on hypergraph transversal property for nodes that validate cross sidechain transactions.
%     For application IoT environments where nodes have varying computing capabilities, the HARB framework proposed a resource manager and an adaptive blockchain module to dynamically assign roles to nodes on the network based on their resource levels. 
    
% \subsubsection{Application layer}
%     The application layer is composed of smart contracts, chaincodes and decentralised applications (DApps).
%     DApps are executed on the client node and are composed of scripts, Application Programming Interfaces (APIs), user interfaces and frameworks.
%     On the other hand, smart contracts and workflows are executed on the endorsing peers. 
%     For data privacy and confidentiality, the HARB framework proposed a Data Tagging and Anonymisation Module (dTAM) as a smart contract.
%     dTAM uses the hypergraph colouring coupled with linkable ring signature and zero-knowledge proofs to achieve the balance between transparency and confidentiality in information exchange.

\subsection{None-Fungible Tokens (NFT)} \label{sec:nft}
The proposed LightweightID manager utilises the NFT tokens for secure and trusted identity of resource constrained IoT devices. 
An IoT device $v_i$ is said to be secure and trusted if it is bound to an NFT $E_i$.
The token structure is described as a tuple to provide a compact representation:
\begin{equation}
    \begin{aligned}
        E_i=<Token ID, Token Name, Device ID,\\ Pseudo ID, Owner ID, Constraints,\\ Issue Time>
    \end{aligned}
\end{equation}
The token structure is blockchain agnostic and can be defined using any standard, including the ERC-721 standard in Ethereum and the Unspent Transaction Output (UTXO) standard in Bitcoin and Hyperledger Fabric.
The token attributes are defined as follows:
\begin{itemize}
    \item \textbf{Token ID:} This is the token identifier composed of hashing three other identifiers (ID), Device ID, Pseudo ID and Owner ID.
    \item \textbf{Token Name:} This is a human-readable descriptive field.
    \item \textbf{Device ID:} This is the ID of a physical IoT device generated by the Physically Unclonable Function (PUF).
    We assume that all IoT devices are capable of implementing PUF.
    \item \textbf{Public Key:} This is a pseudo-identifier of the IoT device on the blockchain platform generated by CL-PKI. 
    \item \textbf{Owner ID:} This field is used in device delegation and ownership management.
    \item \textbf{Constraints:} Contains a number of flags used to validate the token, whether revoked, delegated, or transferred.
    \item \textbf{Issue Time:} This is a timestamp of when the token was issued.
\end{itemize}


\subsection{Constraint Satisfaction Problems (CSP)}\label{sec:csp}
A CSP $P$ is formally described by a triplet $P=(V,D,C)$ where $ V=\left \{ v_{1},v_{2}, \cdots v_{n}\right \}$  is a finite set of variables with $n=|V|$ being the number of variables to be solved in the problem, $ D=\left \{ d_{1},d_{2}, \cdots d_{n}\right \} $  is a finite set of domains for variables in $V$, and $C=\left \{ c_{1},c_{2}, \cdots c_{m}\right \}$ is a set of constraints.
Each constraint $c\in C$ is a pair  $c=\left ( s,\rho  \right )$ where $s\subseteq V$ is a subset of variables, called the scope, and $\rho \subseteq D^{s}$ is a set of assignment functions from the scope of $c$ to the domain of $P(D)$, called the relation of $c$.

There are a variety of constraints in CSP, including unary, binary, and high-order, among others \cite{Brailsford1999}.
Unary constraints involve a single variable (i.e. $v\neq0$).
Binary constraints involve pair of variables.
High-order constraints involve three or more variables.
The aim is to find an assignment $\rho: V\rightarrow D$ of every variable $v_{i} \in V$ from the domains $d_{k} \in D$ in such a way that none of the constraints $c \in C$ is violated.
An assignment $\rho(s)$ is said to be satisfied if for all constraints $\forall \left ( s,\rho  \right )\in C$ there is an assignment function $\rho \in D^{s}$.

Graph-theoretical notation can describe the structural properties of CSP networks in which nodes represent variables and arcs represent constraints.
Most problems are represented as binary CSP, where the constraints involve pairs \cite{Zabih1990}.
A binary CSP has an associated constraint graph $P=(V,E)$, where $V$ is a set of variables, and $E=\{ \left ( s_{i} ,\rho  \right )| s=\left ( v_{i},v_{j} \right )$ is a set of binary constraint relations between $ v_{i}$ and $v_{j}$ for all $v_{i}\wedge v_{j} \in V\}$.
However, the binary constraint graph hides the contextual interaction information, particularly the tightness of the constraints.
Consequently, the standard notation of hypergraphs can be adopted to represent high-order relationship constraints.

A hypergraph is a pair $H=(V, E)$, where $V$ is an arbitrary set of variables, and $E$ is a set of subsets of variables $V$, called hyperedges \cite{Karumba2020}.
For any CSP instance $P$, its associated constraint hypergraph is a graph $P  =  \left ( V,E,C \right )$, where $V$ is a set of variables, $E$ is a set of domains, and $C=\{ \left ( s_{i} ,\rho  \right )| s_{i}=(v_{1},v_{2},v_{3},\dots,v_{t})\}$ is a set of constraints.
Each constraint $c \in C$ is a high-order relation  on $s_{i}$ given the assignment function $\rho(s_{i})$. 

Next, in \cref{sec:plexichain}, we present the proposed PlexiChain framework that implements the security requirement and the proposed design goals based on blockchain and CSP to address the security threats and vulnerabilities identified in this section.

==> sections/5-performance_evaluation.tex <==
\section{Performance Evaluation} \label{sec:performance_evaluations}
This section covers the security analysis and performance evaluation of PlexiChain.
First, we describe the base logic of our implementation architecture and the underlying technologies used to implement the proposed solutions.
Then, using a real-world dataset, we conducted a security analysis of the proposed CSP Aggregator Model.
Finally, using the Hyperledger Caliper\footnote{\url{https://hyperledger.github.io/caliper/}} framework, we evaluated the performance of the lightweight MSP component and benchmarked it against the HLF's MSP.

% \begin{figure*}[!th]
%     \centering
%     \includegraphics[width=\linewidth]{figures/plexichain_testbed.png}
%     \caption{Implementation testbed}
%     \label{fig:testbed}
% \end{figure*}

\subsection{Experiment Setup} \label{sec:implementation}
The testbed shown in \Cref{fig:testbed} is running 4 edge nodes and 2 fog nodes of the implemented system model discussed in \Cref{sec:system_model}.
We have deployed the edge nodes on Raspberry PI 4's with 8GB LPDDR4-3200 SDRAM, a Broadcom BCM2711, and Quad-core Cortex-A72 (ARM v8) 64-bit system on chip with 1.5 GHz frequency.
Each Raspberry PI represents a smart meter equipped with a local controller to send energy consumption data from a prosumer building and receive control commands from the aggregator platform. 
The fog nodes are deployed on two devices: a MacBook Pro with 8 GB memory and Dual-Core Intel Core i5 with 2.3 GHz frequency; and a Digital Ocean droplet with 8 GB memory and 4vCPUs with 2.4 GHz frequency each.
Each Fog node runs the implemented PlexiChain framework on a docker platform. 

Docker\footnote{\url{https://docs.docker.com/get-started/overview/}} is a set of platform-as-a-service products that use OS-level virtualization to deliver microservices in packages called containers.
First, we describe and configure each PLexiChain component (i.e. peers, orderers, KGC, and committers) as a micro-service in a docker-compose (version 3.0) script.
Compose\footnote{\url{https://docs.docker.com/compose/}} is a tool for defining and running multiple docker containers.
At the application layer, we used Node-Red\footnote{\url{https://nodered.org/}} to implement the DF Trading DApp.
Node-Red is a programming tool for connecting hardware devices (e.g. sensors, smart meters, and flexible resources), APIs and other online services.
We used the HARB framework to implement the blockchain network components at the consensus layer, including peers, orderers, MSP, and chaincodes.
We utilized HARB's modular design to plug in the proposed lightweight MSP at the network layer.
Lastly, all smart contracts are implemented using the golang programming language.

\subsection{Results and Discussions}
This section evaluates the PlexiChain framework and benchmarks it against the certificate-based HLF framework as our baseline.
Recall that one of the key contributions of PlexiChain is to reduce the high computation and communication costs incurred during certificate management.
To evaluate this, we compare our framework's memory footprint, transactions throughput, and computing latency with that of the baseline.
Throughput is defined as the rate at which transactions are processed after being received.
Latency is the time taken from when a transaction is issued to the time it is committed.
We use Hyperledger Caliper, a benchmarking tool for blockchain frameworks, to evaluate the two Systems Under Test (SUT). 


\begin{figure}[!h]
    \centering
    \subfigure[Memory Footprint]{
        \includegraphics[width=.45\linewidth]{figures/eval_memory.png}
        \label{fig:eval_memory}
    }
    \subfigure[Throughput and Latency]{
        \includegraphics[width=.45\linewidth]{figures/eval_combo.png}
        \label{fig:eval_throughput_latency}
    }
    \caption{Performance Evaluation}
    \label{fig:results}
\end{figure}

\subsubsection{Memory footprint}
To evaluate the memory footprint, we implement the key generation phase algorithms of PlexiChain and the baseline in the Caliper's workload configuration file.
The workload configuration file implements the business logic to emulate a SUT client.
We then configure the caliper benchmark configuration file to send a workload simulating credential generation for devices in groups of 20, 40, 60, 80 and 100 to the SUT.
The benchmark configuration executes the workload configuration and collects results.
The results show that our framework reduces the amount of memory used by about 33.33\%, as shown in \Cref{fig:eval_memory}.
The lightweight MSP only stores the partial private keys for each device required to generate the private-public key pair, while the baseline MSP stores both the certificate and the public-private key pair for all devices.

\subsubsection{Throughput and Latency}
We implement the transaction signing phase of both PlexiChain and baseline to evaluate throughput and latency in a new caliper workload configuration file.
Then, we configure the benchmark configuration file to execute the workload by sending transactions to the SUT at a send rate of 20, 40, 60, and thorough 200 transactions per sec (tps). 
\Cref{fig:eval_throughput_latency} shows a comparison of latency and throughput between PlexiChain and the baseline. 
Throughput results show that for the given transactions range, the baseline reaches saturation point at 120tps,  while that of PlexiChain is higher than 170tps.
PlexiChain improves throughput because the transaction size is much smaller than the baseline, including a certificate for signing key verification.
Similarly, latency in PlexiChain significantly reduces compared to the baseline, especially at higher transaction rates.
Note that latency increases exponentially after the baseline reaches the throughput saturation point.
This is because Caliper does not have a queuing mechanism, and thus the transactions start to fail.
